Lunar Crater Identification via Deep Learning

Crater counting on the Moon and other bodies is crucial to constrain the dynamical history of the Solar System. This has traditionally been done by visual inspection of images, thus limiting the scope, efficiency, and/or accuracy of retrieval. In this paper we demonstrate the viability of using convolutional neural networks (CNNs) to determine the positions and sizes of craters from Lunar digital elevation maps (DEMs). We recover 92% of craters from the human-generated test set and almost double the total number of crater detections. Of these new craters, 15% are smaller in diameter than the minimum crater size in the ground-truth dataset. Our median fractional longitude, latitude and radius errors are 11% or less, representing good agreement with the human-generated datasets. From a manual inspection of 361 new craters we estimate the false positive rate of new craters to be 11%. Moreover, our Moon-trained CNN performs well when tested on DEM images of Mercury, detecting a large fraction of craters in each map. Our results suggest that deep learning will be a useful tool for rapidly and automatically extracting craters on various Solar System bodies. We make our code and data publicly available at https://github.com/silburt/DeepMoon.git and https://doi.org/10.5281/zenodo.1133969 .

==> oldbibliography <==
\begin{thebibliography}{00}

\bibitem{1} Emami E., Bebis G., Nefian A., Fong T. (2015) Automatic Crater Detection Using Convex Grouping and Convolutional Neural Networks. In: Bebis G. et al. (eds) Advances in Visual Computing. Lecture Notes in Computer Science, vol 9475. Springer, Cham

\bibitem{2} Stepinski, T. F., Wei Ding, and R. Vilalta. "Detecting impact craters in planetary images using machine learning." Intelligent Data Analysis for Real-Life Applications: Theory and Practice, IGI Global (2012): 146-159.

\bibitem{3} Salamuni{\'c}car, G., \& Lon{\v c}ari{\'c}, S.\ 2010.\ Method for crater detection from martian digital topography data using gradient value/orientation, morphometry, vote analysis, slip tuning, and calibration.\ IEEE Transactions on Geoscience and Remote Sensing 48, 2317-2329.

\bibitem{4} Wetzler, P., Honda, R., Enke, B., Merline, W., Chapman, C., \& Burl, M. (2005). Learning to detect small impact craters. Seventh IEEE Workshops on Application of Computer Vision., 1, pp. 178-184. Breckenridge.

\bibitem{5} Cohen, J.P., Lo, H.Z., Lu, T., Ding, W., 2016. Crater Detection via Convolutional Neural
Networks. In: Proceedings of the 47th Lunar and Planetary Science Conference,
Abstract \# 1143.

\bibitem{6} Palafox, Leon F., et al. "Automated detection of geological landforms on Mars using Convolutional Neural Networks." Computers \& Geosciences 101 (2017): 48-56.

\bibitem{7} Bandeira, Louren�o, Wei Ding, and Tomasz F. Stepinski. "Detection of sub-kilometer craters in high resolution planetary images using shape and texture features." Advances in Space Research 49.1 (2012): 64-74.

\bibitem{8} Zhang, Yingying, et al. "Single-image crowd counting via multi-column convolutional neural network." Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition. 2016.

\bibitem{9} Zeng, Lingke, et al. "Multi-scale Convolutional Neural Networks for Crowd Counting." arXiv preprint arXiv:1702.02359 (2017).

\bibitem{10} Krizhevsky, Alex, Ilya Sutskever, and Geoffrey E. Hinton. "Imagenet classification with deep convolutional neural networks." Advances in neural information processing systems. 2012.

\bibitem{11} Ciregan, Dan, Ueli Meier, and J�rgen Schmidhuber. "Multi-column deep neural networks for image classification." Computer Vision and Pattern Recognition (CVPR), 2012 IEEE Conference on. IEEE, 2012.

\bibitem{12} Long, Jonathan, Evan Shelhamer, and Trevor Darrell. "Fully convolutional networks for semantic segmentation." Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition. 2015.

\bibitem{13} Ronneberger, Olaf, Philipp Fischer, and Thomas Brox. "U-net: Convolutional networks for biomedical image segmentation." International Conference on Medical Image Computing and Computer-Assisted Intervention. Springer, Cham, 2015.

\bibitem{14} LeCun, Yann, et al. "Backpropagation applied to handwritten zip code recognition." Neural computation 1.4 (1989): 541-551.

\bibitem{15} Kingma, Diederik, and Jimmy Ba. "Adam: A method for stochastic optimization." arXiv preprint arXiv:1412.6980 (2014).

\bibitem{16} Srivastava, Nitish, et al. "Dropout: a simple way to prevent neural networks from overfitting." Journal of machine learning research 15.1 (2014): 1929-1958.

\bibitem{17} Greeley, Ronald, and Donald E. Gault. "Precision size-frequency distributions of craters for 12 selected areas of the lunar surface." Earth, Moon, and Planets 2.1 (1970): 10-77.

\bibitem{18} Kirchoff, M., K. Sherman, and C. Chapman. "Examining lunar impactor population and evolution: Additional results from crater distributions on diverse terrains." EPSC-DPS Joint Meeting 2011. 2011.

\bibitem{19} Robbins, Stuart J., et al. "The variability of crater identification among expert and community crater analysts." Icarus 234 (2014): 109-131.

\bibitem{20} Abadi, Mart�n, et al. "Tensorflow: Large-scale machine learning on heterogeneous distributed systems." arXiv preprint arXiv:1603.04467 (2016).

\bibitem{21} Chollet, Fran\c{c}ois et al. "Keras." Github (2015) \url{https://github.com/fchollet/keras}

\bibitem{22} Van der Walt, Stefan, et al. "scikit-image: image processing in Python." PeerJ 2 (2014): e453.

\bibitem{23} Yu, Fisher, and Koltun, Vladlen. "Multi-Scale Context Aggregation by Dilated Convolutions". Computing Research Repository, arXiv preprint arXiv:1511.07122 (2015). 

\bibitem{24} Abadi, Martín, et al. "Tensorflow: Large-scale machine learning on heterogeneous distributed systems." arXiv preprint arXiv:1603.04467 (2016).

\bibitem{25} Gal, Yarin, and Zoubin Ghahramani. "Dropout as a Bayesian approximation: Representing model uncertainty in deep learning." international conference on machine learning. 2016.

\bibitem[Di et al.(2014)]{dili} Di, K., Li, W., Yue, Z., Sun, Y., Liu, Y.\ 2014.\ A machine learning approach to crater detection from topographic data.\ Advances in Space Research 54, 2419-2429. 


\bibitem[Chung et al.(2014)]{chungchung} Chung, C. P., Chung, O. C., Yam, C. H.\ 2014.\ Lunar Crater Identification from Machine Learning Perspective.\ Acta Futura 9 (2014) 41-45.


\bibitem[Thorey(2015)]{thorey} Thorey, C.\ 2015.\ Detection of lunar floor-fractured craters using machine learning methods.\ European Planetary Science Congress 2015, id.EPSC2015-95 10. 

\bibitem[Boukercha et al.(2014)]{boukercha} Boukercha, A., Al-Tameemi, A., Grumpe, A., W{\"o}hler, C.\ 2014.\ Automatic Crater Recognition Using Machine Learning with Different Features and Their Combination.\ Lunar and Planetary Science Conference 45, 2842. 

\bibitem[Simonyan and Zisserman(2014)]{simon} Simonyan, K., Zisserman, A.\ 2014.\ Very Deep Convolutional Networks for Large-Scale Image Recognition.\ ArXiv e-prints arXiv:1409.1556. 

\bibitem[Szegedy et al.(2014)]{gedy} Szegedy, C., Liu, W., Jia, Y., Sermanet, P., Reed, S., Anguelov, D., Erhan, D., Vanhoucke, V., Rabinovich, A.\ 2014.\ Going Deeper with Convolutions.\ ArXiv e-prints arXiv:1409.4842. 

\bibitem[Gomes et al.(2005)]{n1} Gomes, R., Levison, H.~F., Tsiganis, K., Morbidelli, A.\ 2005.\ Origin of the cataclysmic Late Heavy Bombardment period of the terrestrial planets.\ Nature 435, 466-469. 


\bibitem[Morbidelli et al.(2005)]{n2} Morbidelli, A., Levison, H.~F., Tsiganis, K., Gomes, R.\ 2005.\ Chaotic capture of Jupiter's Trojan asteroids in the early Solar System.\ Nature 435, 462-465. 


\bibitem[Tsiganis et al.(2005)]{n3} Tsiganis, K., Gomes, R., Morbidelli, A., Levison, H.~F.\ 2005.\ Origin of the orbital architecture of the giant planets of the Solar System.\ Nature 435, 459-461. 

\bibitem[Salamuni{\'c}car et al.(2014)]{sala+14} Salamuni{\'c}car, G., Lon{\v c}ari{\'c}, S., Grumpe, A., \& W{\"o}hler, C.\ 2014.\ Hybrid method for crater detection based on topography reconstruction from optical images and the new LU78287GT catalogue of Lunar impact craters.\ Advances in Space Research, 53, 1783-1797.

\bibitem[Met Office (2015)]{cartopy} Met Office. "Cartopy: a cartographic python library with a matplotlib interface." SciTools (2015) \url{http://scitools.org.uk/cartopy/}

\bibitem[LOLA Science Team (2014)]{lola14}LOLA Science Team.\ "LRO LOLA Elevation Model 118m (LDEM GDR)."  USGS Astrogeology Science Center (2014) \url{https://astrogeology.usgs.gov/search/details/Moon/LRO/LOLA/Lunar_LRO_LOLA_Global_LDEM_118m_Mar2014/cub}

\end{thebibliography}
